Trust, Because You Can't Verify:Privacy and Security Hurdles in Education Technology Acquisition Practices

The education technology (EdTech) landscape is expanding rapidly in higher education institutes (HEIs). This growth brings enormous complexity. Protecting the extensive data collected by these tools is crucial for HEIs as data breaches and misuses can have dire security and privacy consequences on the data subjects, particularly students, who are often compelled to use these tools. This urges an in-depth understanding of HEI and EdTech vendor dynamics, which is largely understudied. To address this gap, we conducted a semi-structured interview study with 13 participants who are in EdTech leadership roles at seven HEIs. Our study uncovers the EdTech acquisition process in the HEI context, the consideration of security and privacy issues throughout that process, the pain points of HEI personnel in establishing adequate protection mechanisms in service contracts, and their struggle in holding vendors accountable due to a lack of visibility into their system and power-asymmetry, among other reasons. We discuss certain observations about the status quo and conclude with recommendations for HEIs, researchers, and regulatory bodies to improve the situation.

==> rq4.tex <==
\section{Challenges in Managing HEI Data Post-acquisition (RQ4):}
As HEIs navigate the post-acquisition complexities of EdTech integration, they are exposed to issues surrounding data ownership, off-boarding procedures, and recourse in the event of privacy breaches. 
We discuss our participants' thoughts on these challenges here.


\subsection{Off-boarding EdTech}
EdTech discontinuation is common, prompting an important question: What happens to the data collected by the vendor?
Common reasons for discontinuation include price increases (P1, P3, P6, and P8), vendor disputes (P5, P6, and P8), and the identification of better tools (P1, P2, and P8).

Regardless of the reason, when services are discontinued, vendors typically initiate an off-boarding process outlined in the contract, which ideally involves erasing all institutional data from their systems and providing a confirmation document.
Vendors however, may not be as cooperative as one might like; P2 complained that:

\q{once you tell them [cloud vendors] you're not buying anything from any of them anymore, they are much less inclined to help you off board... it might be as little as half of the off boardings we get the confirmation that. Yes, everything's shut down and all [the university's] data is gone}

While vendors may be contractually obliged to provide a ``written assurance'' (P5) about data erasure, universities need to pursue vendors for assurance, especially for sensitive data. 
P2 went on explaining:

\q{Unless it's in the contract, unless we want to pursue long squabbles with a disinterested party, we essentially have to come to a conversation. If we had 200,000 of our alumni with all their Social Security numbers on it, you can bet we're going to pursue it. If we have 200,000 people with their addresses and a phone number, we're likely to pursue it. If we have 1000 people and it's just their first name, we're probably going to write it off.}

P12 emphasized that while a signed assurance provides ``some legal protection,'' it may not fully address concerns if data remains with the vendor despite claims of erasure.
P5 shared that due to vendors' non-cooperation, the off-boarding for complex systems could take multiple years. 
P3 highlighted a trend towards centralized systems managing various functions from ``student information systems to HR to finance.'' 
They expressed concerns if institutions wish to move away from such integrated systems:

\q{once you get there, it's going to be harder to get off and go anywhere else because you've got one integrated system. There are advantages to that, but then you're locking yourself in and it gets harder to break yourself away.}

Similar to data ownership, contractual language becomes key during off-boarding process, yet, concerns regarding vendor integrity emerge.

\subsection{Handling Privacy Violations}
Privacy incidents, such as data breaches or vendors misusing data, are becoming commonplace in the EdTech space~\cite{edtech_breach_article}. 
P9 identified the large number of EdTech tools per institution---ranging from hundreds to an upwards of thousand services---as one of the major causes of privacy issues:

\q{We deal with so many vendors like probability says someone's going to get [a leak in data]... it's a knotted up ecosystem}

P2 shared that the proliferation of sub-vendors, with inadequate resources, exacerbates the risks of sub-vendor breaches. 

\noindent\textbf{Actions and Accountability.}
Regardless of the cause, privacy incidents leave HEIs with little recourse, as P11 stated:

\q{So, it's a violation. What's the remedy? Because how consoled are you if we don't know till after the fact? Your data is already gone.}

In many cases, HEIs make public announcements about the incident, because it is either legally required to give  ``specific notifications'' (P3) based on the data lost or to control reputational damage.  
P2 stated:

\q{there's also just the business part of making sure that our community feels safe and the reputation in the university is known as a place where you can trust to give and provide data and trust that we're going to take care of it }

In the event of privacy violations, contracts play a vital role in establishing vendors' obligations regarding public notification, legal recourse, damage assessment, and ensuring prevention of future incidents.
However, as P5 noted ``that's [contract] the most serious leverage we can have.'' 
Similarly, P1 told us that ``if they [vendor] committed to maintaining the data privacy, then that's the contractual obligation that there's not much we can do from that standpoint.''

% However, as P3 noted, HEIs encounter limitations in exerting power over vendors despite having contracts in place:

% \q{We are at the mercy of what they do. We don't have the audit ability to be able to go out and make sure that they've secured our environments, our particular instances of our software, or their software that's holding our data.}

\noindent\textbf{Collaborative Information Sharing.}
In the context of addressing privacy incidents, P3 described how they use their collaboration with other universities to help inform them of vendors issues and how to make vendors follow necessary obligations:

\q{We had an incident in the recent past [with data leakage] that we, let's just say leveraged the REN-ISAC that the community is sharing such that others were made aware of some of the issues of this third party. So not only do we leverage the contract and enforce upon the vendor their obligations to notify other institutions that may have been impacted and notify students that may have been impacted but also leverage that community network that we have to help inform others so that they know the extent of what's happened}

\noindent\textbf{Legal Implications and Ambiguous Liability.}
Privacy incidents can carry significant legal repercussions and hefty fines, particularly if they involve protected data, as discussed by P11:
\q{the fines around healthcare records are really scary. Our CISO told us that if they captured all of our healthcare records, he thought it would be about a \$50 million fine.}

Determining liability in such incidents can be challenging, particularly when considering whether the university or the affected vendor should be held accountable.
This challenge is exacerbated if sub-vendors are involved, given that their contract with the primary vendor and data flow between them is invisible to the university. 
P11 expressed their frustrations regarding this ambiguity:

\q{Is it the university [who is liable]? Is it the vendor of the university? Is it the sub vendor or the sub sub vendor? Who is liable? To date, the Department of Education and some very, very sketchy advice says ultimately the university runs the application, they're liable.}

While contracts help to some extent in cases of privacy violations, the need for clearer guidelines and accountability mechanisms become crucial in navigating these situations.


% HEIs are concerned about improper use of data by vendors, and they use the contracts to restrict such uses, as P3 said:
% \q{[A vendor] backed off of what they were doing [using student data] a number of years ago because of concerns raised in the higher-ed space around the privacy associated with students' data. So, I understand the use and make sure that we're protected via contracts. you know, from unintended use that we have not agreed to.}

% P12 also discussed how the written assurance can only go so far after an institution finds out about their data still being with a vendor:

% \q{The signed document creates some legal protection, right? Well, [the vendor] told us that [they] erase[d] [university's data]. So how did they get it over here. But that's going to be an after the fact... [the data is] still out there}

% As P2 stated:

% \q{a cloud entity and then a subsidiary of the cloud entity has a breach. So we had a case where we had a vendor who then had their own vendor and the sub vendor had a breach, but it was our people}
